Generative Pretrained Embedding and Hierarchical Irregular Time Series Representation for Daily Living Activity Recognition

Within the evolving landscape of smart homes, the precise recognition of daily living activities using ambient sensor data stands paramount. This paper not only aims to bolster existing algorithms by evaluating two distinct pretrained embeddings suited for ambient sensor activations but also introduces a novel hierarchical architecture. We delve into an architecture anchored on Transformer Decoder-based pre-trained embeddings, reminiscent of the GPT design, and contrast it with the previously established state-of-the-art (SOTA) ELMo embeddings for ambient sensors. Our proposed hierarchical structure leverages the strengths of each pre-trained embedding, enabling the discernment of activity dependencies and sequence order, thereby enhancing classification precision. To further refine recognition, we incorporate into our proposed architecture an hour-of-the-day embedding. Empirical evaluations underscore the preeminence of the Transformer Decoder embedding in classification endeavors. Additionally, our innovative hierarchical design significantly bolsters the efficacy of both pre-trained embeddings, notably in capturing inter-activity nuances. The integration of temporal aspects subtly but distinctively augments classification, especially for time-sensitive activities. In conclusion, our GPT-inspired hierarchical approach, infused with temporal insights, outshines the SOTA ELMo benchmark.

==> IV._Related_Works_v3_.tex <==
\section{Related Works}

\subsection{Human Activity Recognition and Pre-trained Embeddings}

Recent advances in deep learning have significantly impacted various fields, including HAR. In HAR, sensor-based deep learning techniques are pertain to Convolutional Neural Networks \cite{singh2017convolutional, mohmed2020employing}, autoencoders \cite{wang2016human}, semantics-based approaches \cite{yamada2007applying}, and sequence models \citep{ghods2019activity2vec}. Despite their efficacy, these methods often struggle with temporal aspects, long-term dependencies, and pattern similarities crucial for recognizing ADLs.

In \cite{huang2023human} Huang et Zhang have employed a transformer architecture \cite{vaswani2017attention} with handcrafted features to classify pre-segmented activities on the Aruba dataset from the CASAS benchmark \cite{cook2012casas}. However, their approach had limitations: it omitted the infrequent "respirate" activity and the "Other" category, which includes unidentified activities that share patterns with recognized ones. Additionally, their model had difficulty distinguishing similar activities like "wash dishes" and "meal preparation," and did not fully utilize deep learning's potential for automatic feature extraction.

Advancements in self-supervised learning and sequence modeling, such as bi-LSTM \cite{liciotti_lstm}, ELMo \cite{bouchabou2021using}, and GPT-2 \cite{10179111}, have influenced HAR. \cite{bouchabou2021using} enhanced bi-LSTM classifiers with a frozen, pre-trained ELMo-based sensor embedding. \cite{10179111} used a GPT-2 architecture for predicting sensor events, but this approach was limited to feature engineering and did not leverage GPT-2's capabilities for classification tasks. Additionally, it lacked extensive analysis of embeddings, attention mechanisms, and ablation studies.

\subsection{Hierarchical Models of Actions}

A hierarchical approach is crucial for modeling human actions and recognizing ADLs in smart homes. Various hierarchical models have been developed using the CASAS dataset \cite{cook2012casas}. For example, \cite{Hong2009PMC} explored ontology models for context-aware activities, and \cite{Asghari2019} used Hierarchical Hidden Markov Models. These methods, however, have limitations in recognizing long-term dependencies.

Hierarchical LSTM models have also been applied to activity recognition with wearable sensors \cite{Wang2020CSSP} and RGB-D videos \cite{devanne2019recognition}. \cite{devanne2019recognition} found that hierarchical structures improved recognition performance by processing more information from longer time windows and better understanding activity relationships, highlighting the importance of multi-level time dependencies.

ADLs, such as cooking or cleaning, can vary significantly daily based on the inhabitant's context and goals. Each activity comprises a sequence of unit actions, as identified in \cite{devanne2019recognition} and \cite{Wang2020CSSP}, organized to achieve a distant goal. Activities may also be interdependent, influencing and relying on each other.

==> V._Discussion.tex <==
\section{Discussion}

\subsection{Summary}

In our study on recognizing daily living activities through ambient sensor classifications within smart homes, we embarked on a comparison of two distinct pretrained embeddings applied to ambient sensor activations. Notably, the Transformer Decoder-based embedding (akin to the GPT design) was shown superior in classification tasks when compared to the ELMo pretrained embeddings. By introducing a hierarchical structure, we aimed to exploit the inherent relationships among activity sequences, thereby refining the classification outcomes. The effectiveness of this approach was evident across all three datasets, with the GPTHAR version standing out especially. Furthermore, the inclusion of an hour-of-the-day embedding subtly yet significantly enhanced classification precision, particularly for activities with time-sensitive natures.

\subsection{Limitations and Future Works}

Our study used pre-segmented data, which restricts the potential application of these algorithms in real-time services. %Furthermore, managing large datasets introduces challenges related to training durations. 
Throughout our experiments, we observed that the transformer architecture resulted in longer training times compared to the LSTM embedding-based architecture. %This necessitates further optimization efforts to prevent excessive training durations. 
Additionally, although we selected datasets that encompass various lifestyle configurations, our evaluation was limited to just three datasets of the CASAS benchmark. This raises potential concerns regarding the wider applicability and generalizability of our conclusions. Broadening the scope of our evaluations to encompass a more diverse range of datasets will be pivotal. This would not only test the model's robustness but also enhance its generalizability across various scenarios and environments. 

%\subsection{Future Works}
Our results show an increase in standard deviation values in datasets Aruba and Milan, with a hierarchical structure. We hypothesize for future works that model stability could be improved by the introduction of normalization layers.
%An exhaustive hyperparameter search could not only bolster results, but also to refine and make the model more efficient. Such optimization would be instrumental in achieving better performance while ensuring computational efficiency. 
Lastly, we see a promising avenue in automated segmentation learning. Moving away from pre-segmented data, investigating methods that allow for more natural and continuous activity recognition could pave the way for more realistic and adaptive models. This would potentially overcome the constraints posed by our current segmentation approach, leading to real-world applicable results.

\subsection{Conclusion}
%In the context of smart homes, our study in recognition of daily living activities  underscores the significant advantages of utilizing pre-trained embeddings, with a particular emphasis on the Transformer Decoder-based approach, for this task. We introduced a robust framework dedicated to enhancing the recognition of ADLs. Our results consistently support the hierarchical methodology, highlighting its proficiency in discerning inter-activity relations. With the integration of temporal data, the framework's performance was notably augmented, especially in datasets characterized by sensor anomalies and noise, demonstrating its potential in distinguishing nuanced activity patterns.
In our smart home study, we highlight the benefits of using Transformer Decoder-based methods as an embedding, for recognising daily living activities. Our framework improves ADL recognition, with results favouring a hierarchical approach that excels in identifying inter-activity relationships. Incorporating temporal data significantly enhanced performance, particularly in noisy datasets.%, showcasing the framework's ability to detect subtle activity patterns.

